Network Flow-Based Refinement for Multilevel Hypergraph Partitioning

We present a refinement framework for multilevel hypergraph partitioning that uses max-flow computations on pairs of blocks to improve the solution quality of a $k$-way partition. The framework generalizes the flow-based improvement algorithm of KaFFPa from graphs to hypergraphs and is integrated into the hypergraph partitioner KaHyPar. By reducing the size of hypergraph flow networks, improving the flow model used in KaFFPa, and developing techniques to improve the running time of our algorithm, we obtain a partitioner that computes the best solutions for a wide range of benchmark hypergraphs from different application areas while still having a running time comparable to that of hMetis.

==> R/makros.tex <==
% anderweitig wiederverwendbare Makros fuer Diss
\usepackage{amsfonts}

% allgemeine mathematische Notation
\newcommand{\ceil}[1]{\left\lceil #1\right\rceil}
\newcommand{\floor}[1]{\left\lfloor #1\right\rfloor}
\newcommand{\abs}[1]{\left| #1\right|}
\newcommand{\seq}[1]{\langle #1\rangle}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\enorm}[1]{\norm{#1}_{2}}
\newcommand{\sumnorm}[1]{\norm{#1}_{1}}
\newcommand{\maxnorm}[1]{\norm{#1}_{\infty}}
\newcommand{\xor}{\oplus}
\newcommand{\set}[1]{\left\{ #1\right\}}
\newcommand{\gilt}{:}
\newcommand{\sodass}{\,:\,}
\newcommand{\setGilt}[2]{\left\{ #1\sodass #2\right\}}
\newcommand{\Def}{:=}
\newcommand{\zvektor}[2]{\left(#1,#2\right)}
\newcommand{\vektor}[2]{\left(\begin{smallmatrix}#1\\#2\end{smallmatrix}\right)}
\newcommand{\condition}[1]{\left[#1\right]}
\newcommand{\binomial}[2]{\binom{#1}{#2}}
\newcommand{\even}{\mathrm{even}}
\newcommand{\odd}{\mathrm{odd}}
\newcommand{\mymod}{\,\bmod\,}
\newcommand{\divides}{|}

\newcommand{\blank}{\Box}
\newcommand{\cross}[2]{\langle #1,#2 \rangle}
\newcommand{\defeq}{\mathrel{:=}}
\newcommand{\hash}{\sym{@}}
\newcommand{\hD}[1][D]{^{(#1)}}
\newcommand{\hed}[1][D]{^{1/#1}}
\newcommand{\Lpal}{L_{\mathrm{pal}}}
\newcommand{\Lparity}{L_{\mathrm{parity}}}
\newcommand{\Lvv}{L_{\mathrm{vv}}}
\newcommand{\pD}[1][D]{^{[#1]}}
\newcommand{\pos}[1]{\mathbf{#1}}
\newcommand{\qs}{\mathord{\Box}}
\newcommand{\mSet}[2]{\left\{#1 \mid #2\right\}}
\newcommand{\s}{\mathord{-}}
\newcommand{\CAce}{\hbox{\mdseries\scshape CAce}}
\newcommand{\sCAce}{\s\CAce}
\newcommand{\CAcs}{\hbox{\mdseries\scshape CAcs}}
\newcommand{\sCAcs}{\s\CAcs}
\newcommand{\CAww}{\hbox{\mdseries\scshape CAww}}
\newcommand{\sCAww}{\s\CAww}
\newcommand{\sC}{\s\hbox{\scshape Chng}}
\newcommand{\sD}{\s\hbox{\scshape Diam}}
\newcommand{\sT}{\s\hbox{\scshape Time}}
\newcommand{\CA}{\hbox{\mdseries\scshape CA}}
\newcommand{\sCA}{\s\CA}
\newcommand{\ST}[1]{\langle #1\rangle}
\newcommand{\sym}[1]{\mathord{\hbox{\texttt{\upshape #1}}}}

% Typen
\newcommand{\nat}{\mathbb{N}}
\newcommand{\natnull}{\mathbb{N}_{0}}
%\newcommand{\natless}[1]{\mathbb{N}_{<#1}}
\newcommand{\natless}[1]{\mathbb{N}_{#1}}
%% \newcommand{\nplus}{\mathbb{N}_+}
\newcommand{\real}{\mathbb{R}}
\newcommand{\rplus}{\mathbb{R}_+}
\newcommand{\rnneg}{\mathbb{R}_*}
\newcommand{\integer}{\mathbb{Z}}
% \newcommand{\intint}[2]{\set{#1,\ldots, #2}}
\newcommand{\intint}[2]{{#1}..{#2}}
\newcommand{\realrange}[2]{\left[#1, #2\right]}
\newcommand{\realrangeo}[2]{\left(#1, #2\right)}
\newcommand{\realrangelo}[2]{\left(#1, #2\right]}
\newcommand{\realrangero}[2]{\left[#1, #2\right)}
\newcommand{\unitrange}[2]{\realrange{0}{1}}
\newcommand{\bool}{\set{0,1}}
%\newcommand{\boolean}{\mathbb{B}}
%\newcommand{\mapping}[2]{#1\rightarrow #2}
\newcommand{\mapping}[2]{{#2}^{#1}}
\newcommand{\powerset}[1]{{\cal P}\left(#1\right)}
\newcommand{\NP}{\mathbf{NP}}
\newcommand{\Bild}{\mathbf{Bild}\:}

% Typannotation
\newcommand{\withtype}[1]{\in#1}

% Wahrscheinlichkeitsrechnung
\newcommand{\prob}[1]{{\mathbf{P}}\left[#1\right]}
\newcommand{\condprob}[2]{{\mathbf{P}}\left[#1\;|\;#2\right]}
\newcommand{\condexpect}[2]{{\mathbf{E}}\left[#1\;|\;#2\right]}
\newcommand{\expect}{{\mathbf{E}}}
\newcommand{\var}{{\mathbf{Var}}}
\newcommand{\quant}[2]{\tilde{#1}_{#2}}

% asymptotische Notation
\newcommand{\whpO}[1]{\tilde{\mathrm{O}}\left( #1\right)}
\newcommand{\Oschlange}{$\tilde{\mathrm{O}}$}
\newcommand{\Ohh}[1]{\mathcal{O}\!\left( #1\right)}
\newcommand{\Oh}[1]{\mathcal{O}\!\left( #1\right)}
\newcommand{\oh}[1]{\mathrm{o}\!\left( #1\right)}
\newcommand{\Th}[1]{\Theta\!\left( #1\right)}
\newcommand{\Thsmall}[1]{\Theta( #1)}
\newcommand{\Om}[1]{\Omega\!\left( #1\right)}
\newcommand{\om}[1]{\omega\!\left( #1\right)}
\newcommand{\Oleq}{\preceq}

% local reference
\newcommand{\lref}[1]{\ref{\labelprefix:#1}}
\newcommand{\llabel}[1]{\label{\labelprefix:#1}}
\newcommand{\labelprefix}{} % later redefined using renewcommand

% Diskussion
\newcommand{\discussionsize}{\small}
\newenvironment{discussion}{\par\discussionsize}{\par}

% open issues
%\marginparwidth5cm
\marginparpush2mm
%\newcommand{\frage}[1]{\makebox[0cm]{$\bigotimes$}\marginpar{\tiny #1}}
%\newcommand{\frage}[1]{{\sf[ #1]}\marginpar{?}}
\newcommand{\frage}[1]{}

\newcommand{\mysubsubsection}[1]{\vspace{2mm}\noindent{\bf #1 }}

% punkt am ende von display math
\newcommand{\punkt}{\enspace .}

% Pseudocode Unterst\"utzung
\newenvironment{code}{\noindent%\sf%
\begin{tabbing}%
\hspace{2em}\=\hspace{2em}\=\hspace{2em}\=\hspace{2em}\=\hspace{2em}\=%
\hspace{2em}\=\hspace{2em}\=\hspace{2em}\=\hspace{2em}\=\hspace{2em}\=%
\kill}{\end{tabbing}}

% 1=pos, 2=llable, 3=caption
\newcommand{\labelcommand}{}
\newcommand{\captiontext}{}
\newsavebox{\codeparam}
\newcounter{lineNumber}
\newenvironment{disscodepos}[3]{%
\renewcommand{\labelcommand}{#2}%
\renewcommand{\captiontext}{#3}%
\sbox{\codeparam}{\parbox{\textwidth}{#3}}%
\begin{figure}[#1]\begin{center}\begin{code}\setcounter{lineNumber}{1}}{%
\end{code}\end{center}\caption{\llabel{\labelcommand}\captiontext}\end{figure}}

\newenvironment{disscode}[2]{\begin{disscodepos}{htb}{#1}{#2}}%
{\end{disscodepos}}

% code in text 
%\newcommand{\codel}[1]{{\sf #1}}
%\newcommand{\codem}[1]{\mathsf{#1}}
\newcommand{\codel}[1]{\mbox{\rm "`#1"'}}
\newcommand{\codem}[1]{\mathrm{#1}}

\newcommand{\id}{\tt}
%\newcommand{\Function} {{\bf Function\ }}
%% \newcommand{\Procedure}{{\bf Procedure\ }}
%% \newcommand{\Process}{{\bf process\ }}
%% \newcommand{\While}    {{\bf while\ }}
%% \newcommand{\Repeat}   {{\bf repeat\ }}
%% \newcommand{\Until}    {{\bf until\ }}
%% \newcommand{\Loop}     {{\bf loop\ }}
%% \newcommand{\Exit}     {{\bf exit\ }}
%% \newcommand{\Goto}     {{\bf goto\ }}
%% \newcommand{\Do}       {{\bf do\ }}
%% \newcommand{\Od}       {{\bf od\ }}
%% \newcommand{\Dopar}       {{\bf dopar\ }}
%% \newcommand{\For}      {{\bf for\ }}
%% \newcommand{\Step}      {{\bf step\ }}
%% \newcommand{\Foreach}      {{\bf foreach\ }}
%% \newcommand{\Rof}      {{\bf rof\ }}
%% \newcommand{\Forall}      {{\bf forall\ }}
%% \newcommand{\To}       {{\bf to\ }}
%% \newcommand{\If}       {{\bf if\ }}
%% \newcommand{\Is}       {:=}
%% \newcommand{\Endif}    {{\bf endif\ }}
%% \newcommand{\Fi}       {{\bf fi\ }}
%% \newcommand{\Then}     {{\bf then\ }}
%% \newcommand{\Else}     {{\bf else\ }}
%% \newcommand{\Elsif}    {{\bf elsif\ }}
%% \newcommand{\Return}   {{\bf return\ }}
%% \newcommand{\Set}      {{\bf set\ }}
%% \newcommand{\Boolean}  {{\bf boolean\ }}
%% \newcommand{\Integer}  {$\integer$}
%% \newcommand{\True}     {{\bf true\ }}
%% \newcommand{\False}    {{\bf false\ }}
%% \newcommand{\Bitand}   {{\bf bitand\ }}
%% \newcommand{\Var}      {{\bf var\ }}
%% \newcommand{\Xor}       {{\bf\ xor\ }}
%% \newcommand{\Not}       {{\bf\ not\ }}
%% \newcommand{\Or}       {{\bf\ or\ }}
%% \newcommand{\Div}       {{\bf\ div\ }}
%% \newcommand{\Mod}       {{\bf\ mod\ }}
%% \newcommand{\End}       {{\bf end\ }}
%% \newcommand{\Endfor}       {{\bf endfor\ }}
%% \newcommand{\Rem}[1]   {{\bf (*~}{\rm#1}{\bf ~*)}}
% rechtsbuendiger Kommentar
%\newcommand{\RRem}[1]   {\`{$\mathbf{(*}$~ }{\rm#1}{~$\mathbf{*)}$}}
\newcommand{\RRem}[1]   {\`{\bf --\hspace{0.5mm}--~}{\rm#1}}
\newcommand{\RRemNL}[1]   {\`{\bf (*~ }{\rm#1}{\bf ~*)}%
{\tiny\arabic{lineNumber}}\stepcounter{lineNumber}}

\newcommand{\At}[1]{\left\langle#1\right\rangle}
\newcommand{\NL}{\`{\tiny\arabic{lineNumber}}\stepcounter{lineNumber}}

% Parallelverarbeitungspseudocode
\newcommand{\iProc}{i_\mathrm{PE}}

% Parameter 1=pos, 2=xsize, 3=filename, 4=llabel, 4=caption
\newcommand{\dissepslong}[5]{\begin{figure}[#1]\begin{center}%
\epsfxsize#2\leavevmode\epsfbox{#3.eps}%
\end{center}\caption{\llabel{#4}#5}\end{figure}}

\newcommand{\dissepspos}[4]{\dissepslong{#1}{#2}{\labelprefix/#3}{#3}{#4}}
\newcommand{\disseps}[3]{\dissepspos{htb}{#1}{#2}{#3}}

% Beweise
\newdimen\endofsize\endofsize=0.5em
\def\endofbeweis{~\quad\hglue\hsize minus\hsize
                 \hbox{\vrule height \endofsize width
\endofsize}\par}
% gibt es in amsmath schon
\newenvironment{myproof}{\begin{proof}}{\endofbeweis\end{proof}}
% \newcommand{\platsch}{\hglue\hsize minus\hsize}


% Macros MA Tobias Heuer

\newcommand{\ALL}{\textsc{All}}
\newcommand{\Dual}{\textsc{Dual}}
\newcommand{\Primal}{\textsc{Primal}}
\newcommand{\ISPD}{\textsc{Ispd98}}
\newcommand{\Literal}{\textsc{Literal}}
\newcommand{\SPM}{\textsc{Spm}}
\newcommand{\DAC}{\textsc{Dac}}

\newcommand{\GoldbergTarjan}{\textsc{GoldbergTarjan}}
\newcommand{\EdmondKarp}{\textsc{EdmondKarp}}
\newcommand{\BoykovKolmogorov}{\textsc{BoykovKolmogorov}}
\newcommand{\IBFS}{\textsc{Ibfs}}

\newcommand{\KaHyPar}[1]{KaHyPar-#1}
\newcommand{\KaHyParConfig}[2]{KaHyPar-#1$_\text{(#2)}$}
\newcommand{\hMetis}[1]{hMetis-#1}
\newcommand{\PaToH}[1]{PaToH-#1}

\newcommand{\FlowVariant}[3]{(#1\text{F},#2\text{M},#3\text{FM})}
\newcommand{\Constant}[1]{\textsc{Constant#1}}


==> experiments/final_flow/final_flow_km1_per_instance_m2_ibfs.tex <==
\KaHyPar{MF} & 7782.51 & 17476.91 & 5643.99 & 15863.75 & 15770.06 & 3038.55 & 6143.73 & 7783.87\\ 
\KaHyPar{CA} & 2.44 & 3.04 & 2.16 & 2.03 & 2.66 & 3.39 & 2.07 & 3.84\\ 
\hMetis{R} & 13.61 & 3.53 & 1.60 & 2.03 & 2.72 & 30.28 & 16.42 & 41.32\\ 
\hMetis{K} & 13.23 & 7.82 & 1.37 & 3.89 & 8.49 & 22.26 & 16.33 & 40.14\\ 
\PaToH{Q} & 8.67 & 11.97 & 7.35 & 10.83 & 11.78 & 8.08 & 6.33 & 15.12\\ 
\PaToH{D} & 14.35 & 19.21 & 13.11 & 15.45 & 17.72 & 15.47 & 11.43 & 24.18\\ 


==> experiments/final_flow/final_flow_km1_per_k_m2_ibfs.tex <==
\KaHyPar{MF} & 1057.93 & 3130.20 & 6032.58 & 9362.55 & 14693.96 & 21893.59 & 31706.57\\ 
\KaHyPar{CA} & 2.27 & 2.57 & 2.80 & 2.68 & 2.48 & 2.24 & 2.05\\ 
\hMetis{R} & 21.38 & 15.92 & 14.47 & 13.63 & 11.35 & 9.63 & 7.80\\ 
\hMetis{K} & 21.63 & 15.15 & 13.61 & 13.49 & 10.52 & 9.30 & 7.83\\ 
\PaToH{Q} & 10.51 & 8.36 & 8.35 & 9.09 & 8.54 & 8.27 & 7.48\\ 
\PaToH{D} & 13.26 & 14.24 & 16.07 & 16.59 & 13.87 & 13.61 & 12.66\\ 


==> experiments/final_flow/final_flow_min_km1_per_instance_m2_ibfs.tex <==
\KaHyPar{MF} & 7542.88 & 16828.15 & 5511.40 & 15236.13 & 15197.60 & 2927.42 & 6010.05 & 7478.06\\ 
\KaHyPar{CA} & 2.22 & 2.80 & 1.92 & 1.85 & 2.46 & 3.33 & 1.74 & 3.91\\ 
\hMetis{R} & 14.40 & 4.75 & 2.76 & 3.88 & 4.17 & 31.20 & 16.37 & 41.92\\ 
\hMetis{K} & 12.92 & 7.77 & 2.17 & 4.78 & 6.91 & 21.51 & 16.23 & 40.45\\ 
\PaToH{Q} & 11.48 & 15.24 & 9.53 & 14.36 & 14.98 & 11.44 & 8.36 & 18.45\\ 
\PaToH{D} & 12.06 & 15.57 & 10.90 & 12.47 & 15.17 & 13.64 & 9.45 & 23.04\\ 


==> experiments/final_flow/final_flow_min_km1_per_k_m2_ibfs.tex <==
\KaHyPar{MF} & 1005.76 & 2985.22 & 5805.19 & 9097.31 & 14352.34 & 21537.33 & 31312.48\\ 
\KaHyPar{CA} & 1.71 & 2.16 & 2.51 & 2.51 & 2.45 & 2.16 & 2.05\\ 
\hMetis{R} & 22.25 & 17.62 & 15.63 & 14.29 & 11.94 & 9.80 & 8.01\\ 
\hMetis{K} & 21.82 & 13.66 & 12.76 & 13.49 & 10.62 & 9.18 & 7.81\\ 
\PaToH{Q} & 14.92 & 12.60 & 11.81 & 11.66 & 10.66 & 9.77 & 8.63\\ 
\PaToH{D} & 8.54 & 10.41 & 13.64 & 14.50 & 12.70 & 12.66 & 11.89\\ 


==> experiments/final_flow/final_flow_running_time_m2_ibfs.tex <==
\KaHyPar{MF} & 55.67 & 504.27 & 20.83 & 61.78 & 119.51 & 97.22 & 27.40 & 110.15\\ 
\KaHyPar{CA} & 31.05 & 368.97 & 12.35 & 32.91 & 64.65 & 68.27 & 13.91 &  67.14\\ 
\hMetis{R} & 79.23 & 446.36 & 29.03 & 66.25 & 142.12 & 200.36 & 41.79 & 89.69\\ 
\hMetis{K} & 57.86 & 240.92 & 23.18 & 44.23 & 94.89 & 125.55 & 35.95 & 111.95\\ 
\PaToH{Q} & 5.89 & 28.34 & 1.89 & 6.90 & 9.24 & 10.57 & 3.42& 4.71\\ 
\PaToH{D} & 1.22 & 6.45 & 0.35 & 1.12 & 1.58 & 2.87 & 0.77 & 0.88\\ 


==> experiments/final_flow/final_flow_running_time_per_k_m2_ibfs.tex <==
\KaHyPar{MF} & 19.75 & 32.89 & 47.52 & 60.38 & 78.51 & 100.34 & 119.15\\ 
\KaHyPar{CA} & 12.68 & 17.16 & 23.88 & 31.01 & 41.69 & 57.35 & 76.61\\ 
\hMetis{R} & 27.87 & 51.59 & 74.74 & 91.09 & 109.13 & 128.66 & 149.34\\ 
\hMetis{K} & 25.47 & 32.27 & 42.50 & 53.41 & 74.00 & 109.12 & 152.92\\ 
\PaToH{Q} & 1.93 & 3.61 & 5.44 & 7.01 & 8.40 & 10.06 & 11.44\\ 
\PaToH{D} & 0.43 & 0.77 & 1.12 & 1.42 & 1.71 & 2.02 & 2.29\\ 


==> experiments/flow_alpha/flow_alpha_effectiveness_table_m2_ibfs2.tex <==
$1$ & -6.06 & -5.52 & 0.23 & 0.24 \\ 
$2$ & -3.15 & -2.06 & 0.55 & 0.73 \\ 
$4$ & -1.89 & -0.19 & 0.86 & 1.20 \\ 
$8$ & -0.87 & 0.96 & 1.20 & 1.69 \\ 
$16$ & -0.29 & 1.66 & 1.52 & 2.17 \\ 
\cmidrule{1-5}% 
Ref. &  \multicolumn{1}{c}{\FlowVariant{-}{-}{+}} & 6377.15 &  &  \\ 


==> experiments/flow_alpha/flow_alpha_modeling_comparison_epsilon_table.tex <==
$1$ & 7.7 & 8.1 & 7.6 & 11.7 & 11.3 & 10.5 \\ 
$2$ & 7.9 & 6.6 & 4.8 & 11.0 & 9.1 & 7.8 \\ 
$4$ & 6.9 & 3.9 & 2.7 & 9.9 & 7.3 & 5.4 \\ 
$8$ & 5.1 & 2.3 & 1.5 & 8.6 & 5.3 & 3.9 \\ 
$16$ & 3.4 & 1.3 & 1.2 & 7.0 & 4.1 & 3.5 \\ 


==> experiments/flow_alpha/flow_alpha_modeling_comparison_table.tex <==
$1$ & -15.48 & -6.09 & -15.26 & -5.60 & 0.14 & 0.23 \\ 
$2$ & -10.50 & -3.19 & -10.12 & -2.07 & 0.36 & 0.73 \\ 
$4$ & -5.98 & -1.82 & -5.08 & -0.19 & 0.67 & 1.21 \\ 
$8$ & -3.22 & -0.85 & -1.64 & 0.98 & 1.25 & 1.71 \\ 
$16$ & -1.52 & -0.19 & 0.51 & 1.75 & 1.87 & 2.21 \\ 
\cmidrule{1-7}% 
Ref. & \multicolumn{2}{c}{\FlowVariant{-}{-}{+}} & \multicolumn{1}{c}{$6373.88$} & &\multicolumn{2}{c}{} \\ 


==> experiments/flow_alpha/flow_alpha_table_m2_ibfs.tex <==
$1$ & -6.09 & 12.91 & -5.60 & 13.40 & 0.25 & 15.03 & 0.23 & 15.16 & 0.54 & 67.90 \\ 
$2$ & -3.19 & 15.75 & -2.07 & 16.74 & 0.59 & 16.98 & 0.73 & 17.51 & 1.11 & 140.24 \\ 
$4$ & -1.82 & 20.37 & -0.19 & 21.88 & 0.90 & 20.43 & 1.21 & 21.53 & 1.66 & 269.63 \\ 
$8$ & -0.85 & 28.49 & 0.98 & 30.67 & 1.24 & 26.51 & 1.71 & 28.68 & 2.20 & 512.12 \\ 
$16$ & -0.19 & 43.32 & 1.75 & 46.66 & 1.60 & 37.51 & 2.21 & 41.31 & 2.76 & 973.91 \\ 
\cmidrule{1-11}% 
Ref. & \multicolumn{2}{c}{\FlowVariant{-}{-}{+}} & 6373.88 & 13.73 & \multicolumn{6}{c}{} \\ 


==> experiments/speed_up_heuristics/heuristic_table_m2_ibfs.tex <==
\KaHyPar{CA} & 7077.20 & 6820.17 & \multicolumn{1}{c}{-} & 29.26 \\ 
\KaHyPar{MF} & 2.47 & 2.12 & 43.04 & 72.30 \\ 
\KaHyParConfig{MF}{S1} & 2.41 & 2.06 & 33.89 & 63.15 \\ 
\KaHyParConfig{MF}{S1,S2} & 2.40 & 2.05 & 28.52 & 57.78 \\ 
\KaHyParConfig{MF}{S1,S2,S3} & 2.41 & 2.06 & 21.23 & 50.49 \\ 

